Probabilistic Population Protocol Models

Population protocols are a relatively novel computational model in which very resource-limited anonymous agents interact in pairs with the goal of computing predicates. We consider the probabilistic version of this model, which naturally allows to consider the setup in which a small probability of an incorrect output is tolerated. The main focus of this thesis is the question of confident leader election, which is an extension of the regular leader election problem with an extra requirement for the eventual leader to detect its uniqueness. Having a confident leader allows the population protocols to determine the convergence of its computations. This behaviour of the model is highly beneficial and was shown to be feasible when the original model is extended in various ways. We show that it takes a linear in terms of the population size number of interactions for a probabilistic population protocol to have a non-zero fraction of agents in all reachable states, starting from a configuration with all agents in the same state. This leads us to a conclusion that confident leader election is out of reach even with the probabilistic version of the model.

==> pages/acknowledgements.tex <==
\makeatletter
\ifthenelse{\pdf@strcmp{\languagename}{english}=0}
{\addcontentsline{toc}{chapter}{Acknowledgments}}
{\addcontentsline{toc}{chapter}{Danksagungen}}
\makeatother
\thispagestyle{empty}

\vspace*{20mm}

\begin{center}
\makeatletter
\ifthenelse{\pdf@strcmp{\languagename}{english}=0}
{\usekomafont{section} Acknowledgments}
{\usekomafont{section} Danksagungen}
\makeatother
\end{center}

\vspace{10mm}

%TODO: Acknowledgments

I would like to thank my supervisor, Javier Esparza, for sparking my interest in theoretical computer science with his one-of-a-kind lectures and incredible explanatory skills. He is the reason why I have mainly taken elective modules and practical courses in this field over my last $3$ semesters at TUM, and now had the opportunity to conduct my own research in this area.

I would also like to thank my advisor, Mikhail Raskin, who gave me all the needed support over the course of writing this thesis. He provided me with a wide range of research topics and made sure that I stuck to the one that matches my interests, strengths and intentions. I am grateful for his quick responses, valuable comments and explanations, and his outstanding ability to spot the core flaws to my yet another sloppy proof sketch in a matter of minutes. I really enjoyed the insightful discussions we had on the topic and beyond. I am looking forward to meeting you in person, Mikhail! 

\cleardoublepage{}


==> pages/cover.tex <==
\begin{titlepage}
  % HACK for two-sided documents: ignore binding correction for cover page.
  % Adapted from Markus Kohm's KOMA-Script titlepage=firstiscover handling.
  % See http://mirrors.ctan.org/macros/latex/contrib/koma-script/scrkernel-title.dtx,
  % \maketitle macro.
  \oddsidemargin=\evensidemargin\relax
  \textwidth=\dimexpr\paperwidth-2\evensidemargin-2in\relax
  \hsize=\textwidth\relax

  \centering

  \IfFileExists{logos/tum.pdf}{%
    \includegraphics[height=20mm]{logos/tum.pdf}
  }{%
    \vspace*{20mm}
  }

  \vspace{5mm}
  {\huge\MakeUppercase{\getFaculty{}}}\\

  \vspace{5mm}
  {\large\MakeUppercase{\getUniversity{}}}\\

  \vspace{20mm}
  {\Large \getDoctype{}}

  \vspace{15mm}
  \makeatletter
  \ifthenelse{\pdf@strcmp{\languagename}{english}=0}
  {\huge\bfseries \getTitle{}}
  {\huge\bfseries \getTitleGer{}}
  \makeatother

  \vspace{15mm}
  {\LARGE \getAuthor{}}

  \IfFileExists{logos/faculty.png}{%
    \vfill{}
    \includegraphics[height=20mm]{logos/faculty.png}
  }{}
\end{titlepage}


==> pages/disclaimer.tex <==
\cleardoublepage{}

\thispagestyle{empty}
\vspace*{0.8\textheight}
\noindent
\makeatletter
\ifthenelse{\pdf@strcmp{\languagename}{english}=0}
{I confirm that this \MakeLowercase{\getDoctype{}} is my own work and I have documented all sources and material used.}
{Ich versichere, dass ich diese \getDoctype{} selbstständig verfasst und nur die angegebenen Quellen und Hilfsmittel verwendet habe.}
\makeatother

\vspace{15mm}
\noindent
\getSubmissionLocation{}, \getSubmissionDate{} \hspace{50mm} \getAuthor{}

\cleardoublepage{}

